On generic supercuspidal representations of $Sp_{2n}$

We will construct a family of irreducible generic supercuspidal representations of the symplectic groups over non-archimedian local field $F$ of odd residual characteristic. The supercuspidal representations are compactly induced from irreducible representations of the hyperspecial compact subgroup which are inflated from irreducible representations of finite symplectic groups over the finite quotient ring of the integer ring of $F$ modulo high powers of the prime element.

==> degree.tex <==
\section{Formal degree of supercuspidal representations}
\label{sec:formal-degree-of-supercuspidal-representation}

